Enhancing a Student Productivity Model for Adaptive Problem-Solving Assistance

Research on intelligent tutoring systems has been exploring data-driven methods to deliver effective adaptive assistance. While much work has been done to provide adaptive assistance when students seek help, they may not seek help optimally. This had led to the growing interest in proactive adaptive assistance, where the tutor provides unsolicited assistance upon predictions of struggle or unproductivity. Determining when and whether to provide personalized support is a well-known challenge called the assistance dilemma. Addressing this dilemma is particularly challenging in open-ended domains, where there can be several ways to solve problems. Researchers have explored methods to determine when to proactively help students, but few of these methods have taken prior hint usage into account. In this paper, we present a novel data-driven approach to incorporate students' hint usage in predicting their need for help. We explore its impact in an intelligent tutor that deals with the open-ended and well-structured domain of logic proofs. We present a controlled study to investigate the impact of an adaptive hint policy based on predictions of HelpNeed that incorporate students' hint usage. We show empirical evidence to support that such a policy can save students a significant amount of time in training, and lead to improved posttest results, when compared to a control without proactive interventions. We also show that incorporating students' hint usage significantly improves the adaptive hint policy's efficacy in predicting students' HelpNeed, thereby reducing training unproductivity, reducing possible help avoidance, and increasing possible help appropriateness (a higher chance of receiving help when it was likely to be needed). We conclude with suggestions on the domains that can benefit from this approach as well as the requirements for adoption.

==> tables/help_apt-def.tex <==
\begin{table}
\centering
\caption{Definition of possible help avoidance, abuse, and appropriateness using HelpNeed}
\label{tab:haaa-def}
\begin{tabular}{|l|l|} 
\hline
Help Behavior Metric                          & Definition                                                                                 \\ 
\hline
Possible
  Help Avoidance       & \begin{tabular}[c]{@{}l@{}}\%steps with observed HelpNeed \\but no hints were 
  requested or received\end{tabular}    \\ 
\hline
Possible
  Help Abuse           & \begin{tabular}[c]{@{}l@{}}\%steps with no
  predicted or observed HelpNeed \\but hints 
  were requested\end{tabular}    \\ 
\hline
Possible
  Help Appropriateness & \begin{tabular}[c]{@{}l@{}}\%steps with
  predicted HelpNeed \\and hints were received\end{tabular}                    \\
\hline
\end{tabular}
\end{table}
